Creating and destroying coherence with quantum channels

The emerging quantum technologies rely on our ability to establish and control quantum systems in nonclassical states, exhibiting entanglement and quantum coherence. It is thus crucial to understand how entanglement and coherence can be created in the most efficient way. In this work we study optimal ways to create a large amount of quantum coherence via quantum channels. For this, we compare different scenarios, where the channel is acting on an incoherent state, on states which have coherence, and also on subsystems of multipartite quantum states. We show that correlations in multipartite systems do not enhance the ability of a quantum channel to create coherence. We also study the ability of quantum channels to destroy coherence, proving that a channel can destroy more coherence when acting on a subsystem of a bipartite state. Crucially, we also show that the destroyed coherence on multipartite system can exceed the upper bound of those on the single system when the total state is entangled. Our results significantly simplify the evaluation of coherence generating capacity of quantum channels, which we also discuss.

==> preamble.tex <==
\usepackage{cite}

\usepackage{amsmath} 
\usepackage{amssymb,amsthm}
\usepackage{mathabx}
\usepackage{mathrsfs}
%\usepackage{iopams}  
%\usepackage{setstack}
\usepackage{bbm}




\usepackage{graphicx}

\usepackage{hhline}
\usepackage{color, verbatim}

\usepackage{thm-restate}


\usepackage[legalpaper, margin=0.5in]{geometry}
\newcommand{\bra}[1]{\langle #1|}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\braket}[3]{\langle #1|#2|#3\rangle}
%inner product
\newcommand{\ip}[2]{\langle #1|#2\rangle}
%outer product
\newcommand{\op}[2]{|#1\rangle \langle #2|}
\newcommand{\Tr}{\textrm{Tr}}
%%%%%%%%%%%%%%%%%%%%%
% NEWTHEOREM        %
%%%%%%%%%%%%%%%%%%%%%
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem*{remark}{Remark}
%\newtheorem*{example}{Example}


%\newcommand{\slocc}{\overset{\underset{\mathrm{SLOCC}}{}}{\longrightarrow}}
\newcommand{\lm}[1]{\mathcal{C}_{l1}(#1)}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\CP}{\text{CP}}
\newcommand{\dep}{\mathcal{D}}
\newcommand{\aLOCC}{\overline{\text{LOCC}}}
\newcommand{\mrm}[1]{\mathrm{#1}}
\newcommand{\zsim}{\overset{\underset{z}{}}{\sim}}
\newcommand{\nzsim}{\overset{\underset{z}{}}{\not\sim}}
\newcommand{\zpsim}{\overset{\underset{z'}{}}{\sim}}
\newcommand{\nzpsim}{\overset{\underset{z'}{}}{\not\sim}}
\newcommand{\no}[1]{$^{#1}$}
\newcommand{\oexpval}[1]{\overline{\expval{#1}}}

